Hyperspherical Embedding for Point Cloud Completion

Most real-world 3D measurements from depth sensors are incomplete, and to address this issue the point cloud completion task aims to predict the complete shapes of objects from partial observations. Previous works often adapt an encoder-decoder architecture, where the encoder is trained to extract embeddings that are used as inputs to generate predictions from the decoder. However, the learned embeddings have sparse distribution in the feature space, which leads to worse generalization results during testing. To address these problems, this paper proposes a hyperspherical module, which transforms and normalizes embeddings from the encoder to be on a unit hypersphere. With the proposed module, the magnitude and direction of the output hyperspherical embedding are decoupled and only the directional information is optimized. We theoretically analyze the hyperspherical embedding and show that it enables more stable training with a wider range of learning rates and more compact embedding distributions. Experiment results show consistent improvement of point cloud completion in both single-task and multi-task learning, which demonstrates the effectiveness of the proposed method.

==> sections/embedding.tex <==
\section{Review of Learning Point Cloud}
Because our work targets the representations learned from the encoders, we start by reviewing the general structure of point cloud models.
Inspired by the success in the 2D field, most approaches for point cloud analysis adopt encoder-decoder or its variant structures.
Various encoders have been designed to process point clouds, but most of them use a symmetric function, such as max pooling, in the last layer to address the permutation issue contained in the unordered point set.
The outputs from the encoder are learned embeddings, and they will be then processed by following decoders to generate predictions.
In multi-task learning, suppose the input point cloud is denoted by $\mathbf{x} \subseteq {\rm I\!R}^3$, and the pipeline can be summarized as follows:
\begin{equation}
  \mathbf{y}_i = D_i(E(\mathbf{x}))
\end{equation}
where $E(.)$ denotes the encoder with a max pooling in the last layer, $D_i(.)$ denotes the decoder for $i$th task, $\mathbf{y}_i$ demotes the prediction for $i$th task, and the output from encoder $E(\mathbf{x})$ is the embedding. The overall architecture is shown in Figure \ref{fig:architecture}.

\textbf{Existing problems}
Most existing encoders learn representations, or embeddings, from large datasets using the end-to-end training. 
This end-to-end learning strategy does not add constraints on the embeddings, and the embedding distribution tends to be sparse as shown by previous works~\cite{wang2017normface,liu2017sphereface}.
However, a sparse embedding distribution increases the possibility of testing inputs accidentally falling into the unseen regions during training due to gaps or holes in the embedding space.
On the contrary, a compact embedding distribution encourages to preserve more information and helps improve the generalization robustness to unseen features~\cite{liu2021learning,wang2020understanding}.
When it comes to the multi-task learning, embeddings from the encoder are shared by different decoders to improve efficiency of models.
Unfortunately, those decoders learned by different task losses may require different embedding distributions, which may lead to optimization conflicts during training, and an unconstrained embedding space makes such issues occur more frequently~\cite{sener2018multi,yu2020gradient}.
In this paper, we focus on point cloud completion in single-task learning and multi-task learning with other semantics tasks, such as classification and segmentation.
We use fully connected layers and cross entropy loss to predict semantic scores, while decoders with more sophisticated structures are used to generate complete point clouds trained using Chamfer Distance~\cite{fan2017point}.


